Tilting Instability of Magnetically Confined Spheromaks

We consider the tilting instability of a magnetically confined spheromak using 3D MHD and relativistic PIC calculations with an application to astrophysical plasmas, specifically those occurring in magnetar magnetospheres. The instability is driven by the counter alignment of the spheromak's intrinsic magnetic dipole with the external magnetic field. Initially the spheromak rotates - tilts - trying to lower its magnetic potential energy. As a result a current sheet forms between the internal magnetic field of a spheromak and the confining field. Magnetic reconnection sets in; this leads to the annihilation of the newly counter-aligned magnetic flux of the spheromak. This occurs on few Alfv\'en time scales. In the case of higher order (second order) spheromak, the internal core is first pushed out of the envelope, resulting in formation of two nearly independent tilting spheromaks. Thus, the magnetically twisted outer shell cannot stabilize the inner core. During dissipation, helicity of the initial spheromak is carried away by torsional Alfv\'en waves, violating the assumptions of the Taylor relaxation theorem. In applications to magnetars' giant flares, fast development of tilting instabilities, and no stabilization of the higher order spheromaks, make it unlikely that trapped spheromaks are responsible for the tail emission lasting hundreds of seconds.

==> upmath.tex <==
%%
%% This is file `upmath.sty'
%%
%% Copyright (1996) Cambridge University Press
%%
%% by Mark A. Reed
%%
%% This package provides 'upright' math (lower-case Greek, A-Z, a-z,
%% punctuation, < >, \ell, \partial) from the AMS Euler fonts EURM/B.
%% When used internaly at CUP, this package substitutes the correct
%% Monotype Times MTMR/B math fonts.
%%
%% Requires the amsbsy.sty and amsgen.sty packages.
%%
%% Bugs (in the case of unchanged files) should be reported to
%% texline@cup.cam.ac.uk
%%
%% This software may only be used in the preparation of journal articles
%% or books or parts of books to be published by Cambridge University Press.
%% Any other use constitutes an infringement of copyright.
%%
%% This file is distributed in the hope that it will be useful,
%% but WITHOUT ANY WARRANTY; without even the implied warranty of
%% MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.
%%
\ProvidesPackage{upmath}[1996/10/20 v1.0 CUP LaTeX2e package]

\RequirePackage{amsbsy}[1995/01/20] % also includes amsgen.sty

% Macro for changing \mathversion's
\providecommand{\mathch}[2]{% Derived from AMSBSY.STY
  \begingroup
  \let\@nomath\@gobble \mathversion{#1}%
  \math@atom{#2}{%
  \mathchoice%
    {\hbox{$\m@th\displaystyle#2$}}%
    {\hbox{$\m@th\textstyle#2$}}%
    {\hbox{$\m@th\scriptstyle#2$}}%
    {\hbox{$\m@th\scriptscriptstyle#2$}}}%
  \endgroup}

\ifCUPmtlplainloaded \else
%
% The following is from Ueur.fd: changed encoding from U to OML.
% This allows to use eurm/b as (more or less) a math italic font.
%
\DeclareFontFamily{OML}{eur}{\skewchar\font'177}
\DeclareFontShape{OML}{eur}{m}{n}{
  <5> <6> <7> <8> <9> gen * eurm
  <10> <10.95> <12> <14.4> <17.28> <20.74> <24.88> eurm10
  }{}
\DeclareFontShape{OML}{eur}{b}{n}{
  <5> <6> <7> <8> <9> gen * eurb
  <10> <10.95> <12> <14.4> <17.28> <20.74> <24.88> eurb10
  }{}
%
\fi

\DeclareMathVersion{upright}
\DeclareMathVersion{boldupright}
\ifCUPmtlplainloaded
  \SetSymbolFont{letters}{upright}    {OML}{mtm}{m}{n}
  \SetSymbolFont{letters}{boldupright}{OML}{mtm}{b}{n}
\else
  \SetSymbolFont{letters}{upright}    {OML}{eur}{m}{n}
  \SetSymbolFont{letters}{boldupright}{OML}{eur}{b}{n}
\fi

\ifCUPmtlplainloaded
% we want mtr(bx)/mt(b)sy in \mathversion upright/boldupright
  \SetSymbolFont{operators}{upright}{OT1}{mtr}{m}{n}
  \SetSymbolFont{symbols}{upright}{OMS}{mtsy}{m}{n}
  \SetSymbolFont{operators}{boldupright}{OT1}{mtr}{bx}{n}
  \SetSymbolFont{symbols}{boldupright}{OMS}{mtsy}{b}{n}
\fi

\DeclareRobustCommand{\mathup}[1]{\mathch{upright}{#1}}
\DeclareRobustCommand{\mathbup}[1]{\mathch{boldupright}{#1}}

% lower-case Greek
\newcommand\ualpha{\mathup{\alpha}}
\newcommand\ubeta{\mathup{\beta}}
\newcommand\ugamma{\mathup{\gamma}}
\newcommand\udelta{\mathup{\delta}}
\newcommand\uepsilon{\mathup{\epsilon}}
\newcommand\uzeta{\mathup{\zeta}}
\newcommand\ueta{\mathup{\eta}}
\newcommand\utheta{\mathup{\theta}}
\newcommand\uiota{\mathup{\iota}}
\newcommand\ukappa{\mathup{\kappa}}
\newcommand\ulambda{\mathup{\lambda}}
\newcommand\umu{\mathup{\mu}}
\newcommand\unu{\mathup{\nu}}
\newcommand\uxi{\mathup{\xi}}
\newcommand\upi{\mathup{\pi}}
\newcommand\urho{\mathup{\rho}}
\newcommand\usigma{\mathup{\sigma}}
\newcommand\utau{\mathup{\tau}}
\newcommand\uupsilon{\mathup{\upsilon}}
\newcommand\uphi{\mathup{\phi}}
\newcommand\uchi{\mathup{\chi}}
\newcommand\upsi{\mathup{\psi}}
\newcommand\uomega{\mathup{\omega}}
\newcommand\uvarepsilon{\mathup{\varepsilon}}
\newcommand\uvartheta{\mathup{\vartheta}}
\newcommand\uvarpi{\mathup{\varpi}}
\ifCUPmtlplainloaded
  \newcommand\uvarrho{\mathup{\varrho}}
  \newcommand\uvarsigma{\mathup{\varsigma}}
\else
  \let\uvarrho\varrho % don't exist in eurm.
  \let\uvarsigma\varsigma
\fi
\newcommand\uvarphi{\mathup{\varphi}}

\newcommand\ubalpha{\mathbup{\alpha}}
\newcommand\ubbeta{\mathbup{\beta}}
\newcommand\ubgamma{\mathbup{\gamma}}
\newcommand\ubdelta{\mathbup{\delta}}
\newcommand\ubepsilon{\mathbup{\epsilon}}
\newcommand\ubzeta{\mathbup{\zeta}}
\newcommand\uboldeta{\mathbup{\eta}}
\newcommand\ubtheta{\mathbup{\theta}}
\newcommand\ubiota{\mathbup{\iota}}
\newcommand\ubkappa{\mathbup{\kappa}}
\newcommand\ublambda{\mathbup{\lambda}}
\newcommand\ubmu{\mathbup{\mu}}
\newcommand\ubnu{\mathbup{\nu}}
\newcommand\ubxi{\mathbup{\xi}}
\newcommand\ubpi{\mathbup{\pi}}
\newcommand\ubrho{\mathbup{\rho}}
\newcommand\ubsigma{\mathbup{\sigma}}
\newcommand\ubtau{\mathbup{\tau}}
\newcommand\ubupsilon{\mathbup{\upsilon}}
\newcommand\ubphi{\mathbup{\phi}}
\newcommand\ubchi{\mathbup{\chi}}
\newcommand\ubpsi{\mathbup{\psi}}
\newcommand\ubomega{\mathbup{\omega}}
\newcommand\ubvarepsilon{\mathbup{\varepsilon}}
\newcommand\ubvartheta{\mathbup{\vartheta}}
\newcommand\ubvarpi{\mathbup{\varpi}}
\ifCUPmtlplainloaded
  \newcommand\ubvarrho{\mathbup{\varrho}}
  \newcommand\ubvarsigma{\mathbup{\varsigma}}
\else
  \newcommand\ubvarrho{\boldsymbol{\varrho}} % don't exist in eurb.
  \newcommand\ubvarsigma{\boldsymbol{\varsigma}}
\fi
\newcommand\ubvarphi{\mathbup{\varphi}}

% A few other upright symbols
\newcommand\upartial {\mathup{\partial}}
\newcommand\ubpartial{\mathbup{\partial}}

\endinput

% End of file `upmath.sty'
